EOS: Automatic In-vivo Evolution of Kernel Policies for Better Performance

Today's monolithic kernels often implement a small, fixed set of policies such as disk I/O scheduling policies, while exposing many parameters to let users select a policy or adjust the specific setting of the policy. Ideally, the parameters exposed should be flexible enough for users to tune for good performance, but in practice, users lack domain knowledge of the parameters and are often stuck with bad, default parameter settings. We present EOS, a system that bridges the knowledge gap between kernel developers and users by automatically evolving the policies and parameters in vivo on users' real, production workloads. It provides a simple policy specification API for kernel developers to programmatically describe how the policies and parameters should be tuned, a policy cache to make in-vivo tuning easy and fast by memorizing good parameter settings for past workloads, and a hierarchical search engine to effectively search the parameter space. Evaluation of EOS on four main Linux subsystems shows that it is easy to use and effectively improves each subsystem's performance.

==> admin.tex <==
\begin{algorithm}
\small
\LinesNumbered
\KwIn{utilization threshold $T_{i}$ for subsystem {i}}
\KwOut{subsystem whose parameters should be enabled}
\For {\texttt{i} $\gets$ \texttt{1} \textbf{to} \texttt{n}} {
	\texttt{util} $\gets$ monitor\_subsystem(LENGTH, \texttt{i}) \;
	\If{\texttt{util} $> T_{i}$}{
		enable\_subsystem\_parameters(\texttt{i}) \;
		\Return \;
 	}
}
\caption{profiler logic}
\label{admin}
\end{algorithm}


==> annotation.tex <==
%\begin{figure*}[t]
%\lstset{float, language={[ANSI]C}, basicstyle=\ttfamily}%, numbers=left, numberstyle=\tiny}%, basicstyle=\scriptsize\tt}
%\begin{lstlisting}
%//sensor representation
%struct disk_sensor {
%unsigned long concurrency;
%unsigned long rw_ratio;
%unsigned long avg_io_size;
%unsigned long avg_disk_distance;
%unsigned long avg_time;
%unsigned long throughput;
%} DS;
%EOS_SENSOR (DS, "disk 20%:20%:20%:50%:50%", 6);

%void collect_disk_stats(void)
%{
%	// collect disk stats, calculate the signature and thoughput from last call to now
%}
%EOS_STATS_UPDATER(collect_disk_stats, "disk");

%struct gendisk* disk;
%// block driver developers use add_disk(struct gendisk*) to register disk into system
%add_disk(disk);
%EOS_PARAM_DYN_CG(disk->queue->nr_requests, disk->disk_name, "nr_requests", "disk", "unsigned long", 64, 4096, "", 0);
%EOS_PARAM_DYN_CG(disk->queue->backing_dev_info.ra_pages, disk->disk_name, "ra_pages", "disk", "unsigned long", 0, 512, "", 0);
%EOS_PARAM_DYN_FG(*(disk->queue), disk->disk_name, "scheduler", "disk", "string", "deadline", "deadline:cfq:noop", "", &elevator_change);
%EOS_PARAM_DYN_CG(*(disk->queue), disk->disk_name, "quantum", "disk", "unsigned int", 0, 128, "scheduler=cfq", &cfq_quantum_updater);

%unsigned long io_util(void) 
%{
%	// disk io utilization 
%	...
%}
%EOS_SYSTEM_UTIL(io_util, "disk", 20);

%\end{lstlisting}
%\caption{Parameter specifications for disk scheduling subsystem.}
%\label{annot}
%\end{figure*}

\begin{figure*}[t]
\centering
%\begin{minipage}{.5\textwidth}
\lgrindfile{codes/annotation.cpp}
%\end{minipage}
\caption{Parameter specifications for disk scheduling subsystem.}
\label{annot}
\end{figure*}


==> api_example.tex <==
\begin{figure*}
\lstset{float, language={[ANSI]C}, numberstyle=\scriptsize\tt}%, basicstyle=\scriptsize\tt}
\begin{lstlisting}
struct eos_param {
    unsigned long addr;
    const char *name;
    const char *subsys;
    const char *type;
    unsigned long min;
    unsigned long max;
    const char *dep;
    unsigned long func;	
};
 
struct eos_sensor {
    unsigned long addr;
    const char *name;
    const char *subsys;
    int mixed;
};

#define __EOS_PARAM_CG(sym, sec, subsys, type, min, max, dep, func)   \
   extern typeof(sym) sym;                                 \
   static const char __kstrtab_##sym[]                     \
   __attribute__((section("__ksymtab_strings"), aligned(1)))       \
   = MODULE_SYMBOL_PREFIX #sym;                            \
   static const struct eos_param __ksymtab_##sym           \
   __used                                                  \
   __attribute__((section("___ksymtab" sec "+" #sym), unused))     \
   = { &sym, __kstrtab_##sym, subsys, type, min, max, dep, func }           

#define EOS_PARAM_CG(sym, subsystem, type, min, max, dep, func)  \
   __EOS_PARAM_CG(sym, "_cg", subsystem, type, min, max, dep, func)



/* corse-grained parameter */
unsigned int sysctl_sched_latency = 6000000ULL;
EOS_PARAM_CG(sysctl_sched_latency, "scheduler", "unsigned int", 1000000, 1000000000, "", 0);

/* fine-grained parameter */
volatile int method_tuner = 0;
EOS_PARAM_FG(method_tuner, "lock", "int", 0, 2, "", 0);

struct disk_sensor {
       unsigned long f1;
       unsigned long f2;	
       unsigned long thp;	
};
struct disk_sensor DS;
EOS_SENSOR(DS, "disk 10%:5%", 3);

\end{lstlisting}
\caption{Examples of using EOS APIs}
\label{ae}
\end{figure*}


==> cases-new.tex <==
\section{Evaluation} \label{eval}

We focus our evaluation on the following three questions:

\begin{enumerate}
\item Is \xxx easy to use?
\item Can \xxx find parameter settings that significantly outperform than
  default?
\item Can \xxx consistently benefit different kernel subsystems?
\end{enumerate}

Each of the next four subsections presents a case study of applying \xxx
to one of the four main non-networking subsystems in the Linux kernel: I/O
scheduling, CPU scheduling, locking, and page replacement subsystems.
% A summary of results is presented in Table~\ref{tab:summary-of-results}.

%% To demonstrate the effectiveness of our proposal, a number of case studies have been 
%% implemented to show how to make the default operating system mechanisms auto-tunable and 
%% how to cache algorithm parameters. Our examples focus on the major subsystems in the Linux 
%% kernel, such as disk scheduling policies and spin locking protocols. For each case study, 
%% we present the target algorithm parameters along with the parameter specification. Then,
%% the metrics used to represent application signatures and subsystem throughput are introduced. 
%% We also detail how to expose the metrics in a light-weight and scalable way in Linux. 
%% Finally, a set of benchmarks are used to evaluate the performance improvements of our system 
%% (with and without \textsc{policy cache}), compared with the default Linux policy and other 
%% competitive policies.  
 
%% \subsection{Experimental Platform}
%% The effectiveness of our proposal has been verified on two platforms. 
%% One is an Intel multi-core system. On the system, one Xeon E5-1620 chip exists and four cores 
%% are accommodated. Hyper-threading technology is supported in the system and each core supports two 
%% hardware threads. The frequency of each core is 3.6GHZ. One 10M bytes last level cache (L3) is 
%% shared by all cores. The chip and memory are connected by the use of Quick Path Interface (i.e., 
%% QPI). The total memory size is 32G and two 2T bytes hard disks exist on our system.

%% The other is an AMD 48-core NUMA system. In this system, 4 Opteron 6168 chips exist and each 
%% chip accommodates 12 cores. Intra-chip cores and chips are connected by internal crossbar and 
%% hyper-transport, respectively. The 64G bytes memory is partitioned into 4 banks, where each bank 
%% connects to one of the 4 chips. There are three 1T bytes hard disks in this system.   

%% To measure performance improvements of disk scheduling and CPU scheduling subsystems, the Intel 
%% platform is used. To benchmark the synchronization subsystem, we use the AMD platform.
%% Note that for disk scheduling subsystem, performance improvements are tested not only on real 
%% hardware, but also in kernel-based virtual machine (KVM).       

\subsection{I/O Scheduling}
\label{diskio}

\textbf{Specifying policies.} In the Linux I/O scheduling system, we
annotated four parameters, previously reported to have large performance
impact~\cite{ibm,disktest}.  The first parameter specifies which
I/O scheduling policy to use for a disk.  The version of Linux we used
supports three policies: (1) completely fair queuing
(``\v{cfq}'')~\cite{linux-io-cfq}, (2) deadline-based
scheduling(``\v{deadline}'')~\cite{linux-io-deadline}, and (3) first-come
first-served(``\v{noop}'')~\cite{linux-io-noop}.  To change this parameter
(method \v{setter} in struct \v{param}), we used Linux's function
\v{elevator\_change}.  The second parameter specifies the maximum number
of requests on a disk queue.  The third parameter specifies how many pages
to read ahead.  The last parameter specifies the time slice allocated to
each process when the I/O scheduling policy is set to \v{cfq}.  To
identify workloads, we used five sensors: the number of the concurrent
processes, the read-write ratio of the requests, the average I/O request
size, the average seek distance between two consecutive disk requests, and
the average time between two consecutive requests.  These sensors capture
typical workload characteristics that significantly affect performance.
We set the optimization target to be the number of sectors read or written
per second.  In total, it took us roughly XXX hours and 50 lines of code
to specify the policies in the I/O subsystem.

%% despite that we are not the developers of the I/O subsystem, 

%% We believe kernel developers of the subsystem can do a better job
%% within a shorter period of time.

%% \textbf{Tunable Parameters}
%% For the disk scheduling subsystem, several parameters are explored. Specifically, 
%% we investigate the type of disk scheduler (i.e., CFQ, DEADLINE or NOOP), the number of requests (i,e, \texttt{nr\_request})
%% and the scheduled quantum for each task queue in the CFQ scheduler (i.e., \texttt{quantum}). We select 
%% these set of parameters because they are found to have relatively large performance 
%% impact~\cite{ibm}~\cite{disktest}. Figure~\ref{spec:disk}
%% presents the parameter specifications used in our experiments, where we can see the detailed 
%% parameter descriptions and dependences. For each parameters presented in the specification, 
%% users can modify the value of the parameter easily by writing into a file, whose location has 
%% been provided in the specification.  

%% \input{disk_sig.tex}
%% \textbf{Exposed Information}
%% Table~\ref{sigdisk} presents the exposed metrics used to characterize the applications and represent
%% disk scheduling throughput. As we can see, one needs to use five metrics to describe the disk scheduling 
%% activities and use the number of read and write sectors per second to represent the throughput. 
%% All these metrics are updated when a disk request is submitted and are exposed to the auto-tuning 
%% module. To ensure the scalability of the updating operation, the exposed information are maintained 
%% in the base of disk. Because the information are written in the kernel, but read at the auto-tuning 
%% module, we use a \texttt{seqlock} to ensure the data consistency. 

\textbf{Experimental setup.} We used an evaluation machine with Ubuntu
13.04 server edition, a quad-core 3.6 GHZ Xeon E5-1620 processor, 32 GB
memory, and two 2 TB hard disks.  We used seven popular I/O benchmarks and
one 12-hour Wikipedia~\cite{wikipedia} I/O trace as the evaluation workloads.
Specifically, the \v{skip} benchmark~\cite{skip} is a micro-benchmark that
starts multiple processes, each of which repeatedly reads 4 KB from a 2 GB
file and skips the following 4KB.  The \v{vskip} benchmark executes
\v{skip} in a KVM virtual machine to evaluate \xxx's performance in a
virtual environment.  The \v{zmIO}~\cite{zmio} benchmark is another
micro-benchmark that starts multiple processes, each of which sequentially
reads 64 KB from a raw disk using direct I/O.  The TPC-B
benchmark~\cite{tpcb} measures the number of executed transactions per
second for a database.  We used PostgreSQL~\cite{postgresql} as the database and
runs TPC-B on another machine.  The table under test was much larger than
the total memory size on our evaluation machine.  The TPC-H
benchmark~\cite{tpch} is a decision support benchmark; we ran four processes
issuing Q2 requests to a PostgreSQL database simultaneously.  The TPC-C
benchmark~\cite{tpcc} evaluates OLTP applications by simulating an environment
where multiple users submit transactions simultaneously into a database.
The vTPC-C executes TPC-C in a KVM virtual machine.  Parallel grep~\cite{taco}
is a macro-benchmarks that uses the GNU \texttt{grep} utility to look for
a non-existent string in the Linux kernel 3.8.8.  Eight processes are
started simultaneously, but each process calls \texttt{grep} in its own
Linux source code copy to reduce the possible kernel lock contentions.
(We only show results of running \v{skip} and TPC-C in a virtual
environment because the other workloads had no difference executing in a
virtual environment or not.)

%% are accommodated. Hyper-threading technology is supported in the system and each core supports two 
%% hardware threads. The frequency of each core is 3.6GHZ. One 10M bytes last level cache (L3) is 
%% shared by all cores. The chip and memory are connected by the use of Quick Path Interface (i.e., 
%% QPI). The total memory size is 32G and two 2T bytes hard disks exist on our system.

 \input{ioschedule.tex}
%% \textbf{Workload Benefits}
%% Seven benchmarks are selected to measure the performance of the disk scheduling subsystem.
%% Specifically, skip~\cite{skip} and zmIO~\cite{zmio} are micro-benchmarks, while TPC-B~\cite{tpcb}, 
%% parallel grep~\cite{taco}, TPC-H~\cite{tpch} and TPC-C~\cite{tpcc} are macro-benchmarks. Note that 
%% benchmarks \textit{vskip} and \textit{vTPC-C} represent we execute skip and TPC-C in the virtual
%% machine. The skip benchmark starts multiple processes and each process repeatedly operates 
%% on a 2G bytes file. Each operation first reads 4K bytes into the private buffer and skips the following 
%% 4K bytes; the zmIO benchmark has each process open another disk for sequential read-only direct I/O. The 
%% reading size is 64K bytes; TPC-B measures the database throughput by the use of executed transactions per 
%% second. We use PostgreSQL as the database and drive this test using pgbench in another client machine. 
%% The operated table size is much larger than the total memorize size; parallel grep is a macro-benchmarks 
%% that uses the GNU \texttt{grep} utility to look for a string in the Linux kernel 3.8.8, which does not exist. 
%% Eight processes are started simultaneously, but each process calls \texttt{grep} in its own Linux source 
%% code copy. Multiple Linux source code copies are used to reduce the possible kernel lock contentions; 
%% TPC-H is a decision support benchmark. We have four processes issue the Q2 request to the PostgreSQL database 
%% simultaneously. The system performance is measured by looking at the execution time; TPC-C benchmarks 
%% the OLTP applications by simulating an environment where multiple users submit transactions simultaneously
%% into the database. The performance is measured by transactions per minute.   

\textbf{Results.} Figure~\ref{disk} shows the performance improvements of
the benchmarks compared to the default setting (deadline in the version of
Ubuntu we used, three other parameters).  With a cold cache, \xxx achieves
over 11$\times$ speedup on \v{skip} and 3$\times$ speedup on parallel \v{grep}.  
Its improvements on other applications are also quite significant, up to 41\%. 
With a warm cache, \xxx gains another 10.0\% on average. Since we designed 
\xxx to handle relatively steady, repeatable workloads, we expect that the 
warm-cache case is more often than cold-cache.

\input{wikitrace.tex}
%\input{hm0.tex}
%\input{web0.tex}
%\input{prn0.tex}
%\textbf{Long Time Running Traces Performance} 
Figure~\ref{tw} presents \xxx's performance on a 12-hour Wikipedia trace.
It outperforms the default policy by over 19.8\% for almost the entire
workload.

%% For each benchmark, the results with cold and hot \textsc{policy cache}
%% are measured.  To compare with our system, the performance of DEADLINE,
%% CFQ and NOOP I/O schedulers are also benchmarked.  For each workload on
%% each I/O scheduler, the workload is executed five times. Except for zmIO,
%% which uses \texttt{/dev/sdb} as the storage, other benchmarks use
%% \texttt{/dev/sda} as the storage.  We report the average, minimal and
%% maximal throughputs normalized to the worst average throughput of
%% DEADLINE, CFQ or NOOP schedulers. Note that the DEADLINE disk I/O
%% scheduler is the default on our testbed. Besides, the performance of the
%% best disk schedulers among DEADLINE, CFQ and NOOP can be regarded as the
%% approximated best performance (We assume the effect of other parameters
%% are not significant).

%% Figure~\ref{disk} presents the performance improvements for seven benchmarks. As can be seen, for 
%% micro-benchmarks skip, vskip and zmIO, AUTO-cold achieves 87.59\%, 106\% and 96.8\% throughput of the best 
%% performed scheduler, respectively. Because DEADLINE I/O scheduler is the default scheduler, one can see the 
%% performance of AUTO-cold is much better than the default for skip (more than 11$\times$). By the use of 
%% \textsc{policy cache}, there is additional performance boost for skip and zmIO. Specifically, AUTO-hot is 
%% able to achieve 96.3\% and 102.1\% throughput of the best scheduler, respectively. One exception is vskip, 
%% which performs worse after the use of \textsc{policy cache}. This happens because in the best cases, DEADLINE 
%% scheduler achieves the same performance of the best performed scheduler (NOOP in vskip) and our system may 
%% select DEADLINE as the best disk I/O scheduler in the auto-tuning phase. However, the large performance 
%% fluctuations in DEADLINE scheduler introduces performance degradation. Compared to the best performed static 
%% schedulers, there are both performance overhead and benefits in our system. In terms of overhead, our 
%% system needs to explore possible parameter configurations to find the best performed one. This will introduce
%% the searching overhead. Although most of the overhead is eliminated after the adoption of parameter cache, 
%% we still need to run the system for one search epoch (five seconds) to collect application signatures, which 
%% are further used to index the \textsc{policy cache}. However, the default parameter settings are usually not 
%% the optimal parameter settings. Thus, overhead still exists. Our system also can bring some performance benefits.
%% Recall that besides the tuning of I/O scheduler type, our system also tunes \texttt{read\_ahead\_kb}, 
%% \texttt{nr\_requests} and \texttt{quantum} of the CFQ scheduler. These tunings may improve performance.   
%% As we can imagine, if benefits are larger than overhead, our system outperforms the best static scheduler, 
%% which is the case in vskip (AUTO-cold) and zmIO (AUTO-hot).  

%% For macro-benchmarks, parallel grep exhibits the best results. AUTO-cold performs nearly the same with the best
%% static IO scheduler CFQ, which produces roughly 3 times more throughput than the default scheduler. Besides, 
%% AUTO-hot delivers a further 10\% performance improvement compared with AUTO-cold. For vTPCC and TPC-H, the 
%% performance improvements are not as large as parallel grep because there is no large performance difference 
%% between all these three static I/O schedulers. However, our system (AUTO-cold) can also provide up to 15\% 
%% and 7\% improvements compared with the best static I/O scheduler, respectively. If we calculate the improvement 
%% percentage with the default scheduler, it appears to be 41.0\% and 13.6\%. In terms of TPC-B, despite almost 
%% the same performance (within 4\%) for all these schedulers, the performance of our system (AUTO-cold and AUTO-hot) 
%% is rather near to the best static scheduler (DEADLINE).       

\input{selected.tex}

Figure~\ref{selected} shows the parameter settings \xxx selected for
each workload.  Note that \xxx may select more than one settings over
repeated executions when the settings have roughly the same performance.
The figure also shows that there is no single scheduling policy that fits
all workload.

%% Figure~\ref{selected} presents the percentage of selecting each disk I/O scheduler as the optimal one for each 
%% benchmark. As we can see, except for vskip, TPC-B and vTPCC, all benchmarks select one I/O scheduler as the best performed 
%% across five experiments. Specifically, in skip and parallel grep, our system selects CFQ; in zmIO, we select DEADLINE; 
%% for TPC-H, NOOP is selected. Combined with the results in Figure~\ref{disk}, we can verify that the selection 
%% is correct. One can also see clearly from this figure that always using one disk I/O scheduler is not the optimal.
%% For the remaining benchmarks, there is a possibility to select different schedulers across five executions. 
%% For vskip and vTPCC, the reason is fluctuated performance for statically configured disk schedulers. As our system
%% selects the best scheduler by executing it for an epoch, this may make the selection wrong, while for TPC-B, 
%% the reason is the performance numbers of DEADLINE and NOOP are rather close. Although a wrong scheduler may be
%% selected in a particular run, most of the time ($>$60\% possibility) we make the correct choice.  

\input{steps.tex}

Figure~\ref{searchtime} shows the time it takes for \xxx to find a good
setting for each workload.  This time ranges from 105 seconds to 145 seconds.

\input{disk_accurate.tex} 

\xxx uses workload signatures to search for settings in the policy cache,
so we also studied the differences and similarities of the signatures of
the evaluated workloads.  Figure~\ref{diska} plots the average seek
distance and the average time between two consecutive disk requests for
the workloads over repeated executions.  These two sensors suffice to
differentiate the workloads.


%% From Figure~\ref{selected}, we can calculate how many search steps are needed for each benchmark on average to find 
%% the optimal parameter settings. The results are presented in Figure~\ref{step}. As 21, 29 and 21 search steps are 
%% acquired to find the the optimal parameter settings for DEADLINE, CFQ and NOOP schedulers, respectively, 29 search 
%% steps are required in skip and parallel grep; 21 steps are needed for vskip, zmIO, TPC-B and TPC-H; 22.6 steps are 
%% needed on average for vTPC-C. 
%% \input{dis.tex}  
%% Another metric to measure the performance of our system is how many AUTO-cold runs are needed before we have a 
%% AUTO-hot execution. The metric indicates that how long we start to reuse the execution history. Figure~\ref{dis} 
%% presents the distribution. As we can see, all benchmarks require at most three 
%% AUTO-cold executions, except for skip, which requires six at most. The difference between skip and other benchmarks 
%% is caused by the relatively short execution time in skip. By looking at our system log information, we find that skip 
%% needs at least two runs to finish the auto-tuning process. Because our system has the feature of continuous search, 
%% which means the latter execution continues the previous search to find the optimal parameter settings if our system 
%% decides that application signatures match a previous execution. However, if application signatures do not match, more 
%% AUTO-cold runs are required, as shown in skip. 



\subsection{CPU Scheduling}
\textbf{Specifying Policies.}  In the CPU scheduling subsystem, we
annotated three parameters. Specifically, \v{sysctl\_sched\_latency\_ns}
specifies the length of time for scheduling each runnable process once.
\v{sysctl\_sched\_min\_granularity\_ns} specifies the minimum time a
process is guaranteed to run when scheduled.
\v{sysctl\_sched\_wakeup\_granularity\_ns}, it describes the ability of
processes being waken up to preempt the current process. A larger value
makes it more difficult preempt the current process~\cite{cfstunable}.  To
identify workloads, we used one sensor: the number of retired instructions
executed in user space. We set the optimization target to be the same.
Overall, we take XXX hours and 36 lines of code to specify the
policy.


%% is the minimal running time
%% of a task when it is scheduled on a CPU. The CFS scheduler adopted in the
%% Linux kernel monitors the number of running tasks (\texttt{nr\_running}).
%% If the inequality $nr\_running >
%% \frac{sysctl\_sched\_latency\_ns}{sysctl\_sched\_min\_granularity\_ns}$
%% holds, \texttt{sysctl\_sched\_latency\_ns} becomes $nr\_running \times
%% sysctl\_sched\_min\_granularity\_ns$.  Otherwise, CFS uses the default
%% \texttt{sysctl\_sched\_latency\_ns} value to execute a round of all
%% running tasks. For the parameter
%% \texttt{sysctl\_sched\_wakeup\_granularity\_ns}, it describes the ability
%% of tasks being waken up to preempt the current task. The larger value
%% means it is more difficult for the task to force the
%% preemption~\cite{cfstunable}. To identify workloads, we used the number of
%% retired instructions at user space as sensor and optimization
%% target. Overall, we take XXX hours and 36 lines of code to specify the
%% policy.
%To provide the instructions executed at user space, we configure the 
%performance monitor unit (PMU) on each CPU to count the retired instruction event and set the event mask to 
%count only user mode instructions. To ensure the scalability when collecting statistics, we maintain the value on a per-CPU 
%basis. At the time of each context switch, the instruction counting data structure on each core is updated. Because 
%it is written in the kernel but read in the auto-tuning module, we use a \texttt{seqlock} to ensure the consistency. At 
%the end of each search epoch, all instruction counting data structures are walked through to report the total. 
    
\input{scheduling.tex}
\textbf{Experimental Setup.}
The evaluation machine is the same to that used to evaluate the disk I/O subsystem. 
To demonstrate the performance improvements of our system, we use the sysbench thread scheduler performance 
test~\cite{sysbench} and five Cilk~\cite{cilk} benchmarks as the workloads. Sysbench starts multiple threads and 
each thread repeatedly locks a mutex, yields the CPU and unlocks the mutex. The execution time is reported at 
end of execution; the Cilk benchmark suite is designed to stress the Cilk programming framework, which is designed 
to parallelize applications based on programmer provided hints. Most of the programs in the suite do a basic 
task, such as merge sort and FFT transformation. All benchmarks are implemented using the interfaces provided 
by the Cilk framework. For each benchmark in each configuration (EOS-cold, EOS-hot and default parameters), 
we report the minimal, maximal and average performance normalized to the worst case. 

\textbf{Results.}
Figure~\ref{scheduling} presents the experimental results of EOS-cold and EOS-hot when compared with the 
results with default parameter settings. As we can see, EOS-cold works well for most programs and the largest 
performance improvement is more than 2$\times$, which comes from the matmul benchmark in Cilk. After the 
use of policy cache, there is further performance boost. The improvement ranges from 3\% to 13$\times$. We 
have analyzed the reason of such significant performance improvements enabled by tuning several CFS parameters. 
For the Cilk benchmarks except FFT, they are affected by the Cilk threading framework. Basically, the framework 
allocates a piece of work to each worker thread. When a thread completes, it tries to steal works from other 
CPUs in a tight loop. This mechanism works well when the number of worker thread is no larger than the number 
of cores. However, if it is not the case, each worker thread executed on a CPU tries to steal a piece of work 
from another CPU after the its own work has been finished. Because the work for each thread is almost the 
same (ensured by the Cilk load balance framework), at some point, all scheduled threads run out of works. 
Then, each work constantly searches jobs from other CPUs and fails. From the view of CPU scheduler, it does 
not know there is no work in all CPUs and should perform a context switch to schedule some tasks with useful 
work. Thus, a lot of CPU cycles are wasted. In contrast, carefully tuning scheduler parameters enables the scheduling of tasks with useful 
work as soon as possible. Thus, this tuning improves performance. 
After detailing the reason of performance improvements, a natural question is what happens if the thread yields its 
CPU to other workers instead of constantly polling? Actually, Cilk framework has already provided this option 
and we use it in the program FFT. Besides, another benchmark sysbench also has the same scheduling policy. Our conclusion 
from measurements indicates that although yielding CPU to other tasks improves the quality of scheduling, it is too 
coarse-grain and using our tuning framework together with this scheduling method still demonstrates performance 
benefits. As we can see from Figure~\ref{scheduling}, there are 40\% and 49\% performance improvements (with 
policy cache) for sysbench and FFT, respectively.

\input{dis_sched}
Next, we continue to evaluate the scheduling subsystem using other two aspects, which are the number of search steps 
and the possibility of hitting policy cache. For search steps, there are no parameter dependencies in the 
parameter specification, so each benchmark needs the same number of search steps to find the optimal parameter configurations. 
By reading the system logs, we found the number is 40. In terms of the second aspect, we present the number 
of eos-cold executions before a eos-hot execution in Figure~\ref{dis_sched}. As we can see, all benchmarks need 
only two eos-cold executions at most, except matmul, which needs four at most, indicating the ease of 
hitting policy cache.
  
\input{sched_accurate}




\subsection{Spin Locking}
\label{syn}

\textbf{Specifying policies.}
In the mixed lock subsystem, two tunable parameters are annotated. One is the \texttt{method\_tuner} 
which is used to invoke protocol switch, the other is \texttt{val\_tuner} which is the polling weight 
in the back-off ticket spin lock ($C$ in Figure~\ref{backoff}). For \texttt{val\_tuner}, it depends heavily 
on the architecture and is hard to determine by experience. Thus, we consider this parameter as a tunable 
as well. For these two parameters, \texttt{backoff\_factor} depends on \texttt{lock\_selector} when it is 
set to be back-off based ticket lock. To identify workloads, we used the average lock acquisition 
time as sensor and use lock acquisitions per second as the optimization target. 
In total it tooks us XXX hours and 30 lines of code to specify the policies in the lock subsystem.

%Another problem of exposing information is which locks should be replaced with our mixed lock. 
%In theory, we can replace each ticket spin lock invocation in the kernel with our locks. In this way, all
%spin locks switch to mixed locks. However, this needs a lot of work in the kernel because 
%the mixed lock interfaces in the current implementation are not compatible with ticket spin locks. 
%Thus, in practice, we only replace the hot locks for each application, which is enough to verify the 
%effectiveness of the mixed lock protocol.      

\textbf{Experimental Setup.}
We use an evaluation machine with Ubuntu 13.04 server edition, eight 48-core 1.9GHZ AMD Opteron processors.
The benefits of mixed lock are demonstrated using two micro-benchmarks (fops and mmapbench) and two 
macro-benchmarks (parallel postmark~\cite{taco} and dbench). The fops benchmark has each process opens its
private file and closes the result; mmapbench has each process map the same continuous 500MBytes with the 
\texttt{MAP\_SHARED} flag from a file, touch each page by reading the first byte, and destroy the mapping. 
Parallel postmark is a multi-threaded benchmark, which has the capability of simulating file servers providing 
email and net news services. Each thread in parallel postmark executes transactions repeatedly on an independent 
set of files (between 0.5 and 10K bytes in size) and each transaction is made up of two steps: (1) creating or 
deleting a file (2) reading or appending a file. Files, file I/O operations and file size are chosen from a 
uniform distribution. To measure the scalability of the Linux kernel instead of I/O, files in the workload 
are created in \textit{tmpfs}. Furthermore, file operations without I/O buffering are used to avoid the 
buffering effect of glibc. Performance is measured by the transaction throughput of all threads. 
Dbench is a multi-process tool used to benchmark the performance of a file system. Based on a user 
provided \texttt{loadfile}, each process is able to do kinds of file operations such as read, write, link, unlink, 
flush, etc. The throughput of these operations are considered as the performance. In our experiments, the 
default \texttt{loadfile} is used and dbench is executed in memory to expose the lock contention bottleneck.  
%In each benchmark, we use mixed lock to replace the hot locks, which are acquired by the use of lock profiling 
%tool \texttt{/proc/lock\_stat}~\cite{lockstat}. Table~\ref{hl} presents replaced hot locks for each benchmark. 

%\input{hlock.tex}
\input{locking.tex}
\textbf{Results.} 
Figure~\ref{lock} presents the performance of our mixed lock implementation with cold and hot cache, 
compared with kinds of synchronization methods including TTAS, back-off based ticket lock, MCS, and the default 
Linux implementation. Note that Linux uses ticket spin lock (without back-off mechanisms) to implement hot locks 
contended in fops, parallel postmark and dbench, but exploits mutex lock for mmapbench. For each synchronization method 
in each benchmark, the measurement is performed five times. In order to create different lock contention level, 
we control the number of tasks used by each benchmark. For example, \textit{fops8} means eight processes are configured 
to execute the fops benchmark. In Figure~\ref{lock}, the average, minimal and maximal throughputs normalized to the 
average throughput of the worst performed synchronization method are presented.      

As can be seen from the figure, for fops (eight processes), mmapbench and parallel postmark, 
eos performs much better than the default Linux implementation (up to 13 times), TTAS and back-off based ticket spin lock. 
This results are expected because implementations such as default Linux and TTAS are only effective for middle level or 
low level lock contention, but when the contention is serious, the scalable lock is able to achieve better performance.
By looking at the logs of our system, we find that the eos cold always selects the MCS lock as the optimal protocol 
for these three benchmarks. This is reasonable because all these three benchmarks experience heavy kernel lock 
contention. When comparing eos with cold cache and hot cache, one can conclude that eos with hot cache always 
performs better than eos cold and the largest improvements can be 4.7\%. As we can imagine, the improvements come from the reduced
searching activities. 
Because all these three benchmarks are lock-intensive, we can actually compare the performance of our system with the 
best implementation, which is MCS for serious lock contention. As can be seen from the figure, eos-hot throughputs 
are rather close to the best case for fops, mmapbench and parallel postmark (101.6\%, 97.2\% and 96.7\% respectively).
The performance differences between eos-hot and MCS are because application signatures are required to further
index the policy cache in our system. However, we need to execute at the default parameter settings to collect the 
information. Thus, if the default settings are not the optimal, which is always the case, the overall performance is 
affected. One point worth mentioning is that the signature collecting overhead can be amortized with the execution of 
application. So, it is negligible for long running applications.  

\input{lock_sele}
For benchmark fops when using two or three processes, we can see the default Linux implementation has the best 
performance. For the two process case, the TTAS lock performs better than back-off based ticket lock and MCS lock.
Thus, our mixed lock selects TTAS as the optimal policy (see Figure~\ref{lock_s}). As we can see, even for eos-cold,
our system performance is rather near to the statically configured TTAS. After the adoption of policy cache, the 
performance has slight improvements. For the three process case, it turns out the back-off based ticket lock 
outperforms other policies and our system can achieve the performance potential after using the policy cache. 
However, as we can see, there is still a performance gap between our system and the default Linux. This gap 
happens because our system has a much more complex lock protocol switching logic than the default Linux's 
lock implementation. This brings overhead when the contention degree is lightweight. 

For dbench, the back-off based ticket lock outperforms MCS lock and the default Linux implementation slightly, 
which are much better than TTAS lock. As indicated in Figure~\ref{lock_s}, our mixed lock can make the correct 
selection all the time and achieve the same performance with back-off based ticket lock.   

We also investigate how consistent of the lock protocol selection by presenting the results of selection across five
experiments in Figure~\ref{lock_s}. As shown in the figure, for each benchmark, all five selections are the same. 
Combined with Figure~\ref{lock}, one can see the selection is correct indeed. Another information that can be received 
from this figure is that always selecting the same lock protocol is not always the optimal. Actually, the results in
this figure verify the correctness of our design: for lightweight contention, TTAS lock should be used; for middle 
level contention, back-off based lock is preferred; for heavy contention, MCS is the best choice. We can also calculate
how many search steps are needed for each benchmark. Basically, we need three search epochs to determine which protocol 
works best, so three steps are need for fops (two and eight processes), mmapbench and parallel postmark. As there is 
another depended parameter when the optimal policy is back-off based ticket lock, 15 search steps are needed for fops 
(three processes) and dbench. 

\input{dis_lock.tex}
Figure~\ref{dis_lock} presents how many eos-cold executions are needed before we encounter an eos-hot run. 
As can be seen from the figure, most benchmarks hits the policy cache at the second execution except for parallel 
postmark and dbench, which require two eos-cold executions. Overall, for the synchronization subsystem, it is rather 
easy to reuse the cached system parameters. 

\input{lock_accurate.tex}
   
\input{memory.tex}

\input{framework}


==> codes/annotation.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{annotation.cpp.lineno}{2014}{5}{1}{8:17}{1388}
\L{\LB{\N{1}\V{:}_\K{struct}_\V{disk\_sensor}_\{}\Tab{30}{\C{}//sensor_representation\CE{}}}
\L{\LB{\N{2}\V{:}}\Tab{7}{\K{unsigned}_\K{long}_\V{concurrency};_\K{unsigned}_\K{long}_\V{rw\_ratio};_\K{unsigned}_\K{long}_\V{avg\_io\_size};}}
\L{\LB{\N{3}\V{:}}\Tab{7}{\K{unsigned}_\K{long}_\V{avg\_disk\_distance};_\K{unsigned}_\K{long}_\V{avg\_time};_\K{unsigned}_\K{long}_\V{throughput};}}
\L{\LB{\N{4}\V{:}_\}_\V{DS};}}
\L{\LB{\N{5}\V{:}_\V{EOS\_SENSOR}_(\V{DS},_\S{}\3disk_20\%:20\%:20\%:50\%:50\%\3\SE{},_\N{6});}}
\index{collect\_disk\_stats}\Proc{collect\_disk\_stats}\L{\LB{\N{6}\V{:}_\K{void}_\V{collect\_disk\_stats}(\K{void})_\{}\Tab{38}{\C{}//_collect_disk_stats,_calculate_the_signature_and_thoughput_from_last_call_to_now\CE{}}}
\L{\LB{\N{7}\V{:}_\}}}
\L{\LB{\N{8}\V{:}}\Tab{7}{\V{EOS\_STATS\_UPDATER}(\V{collect\_disk\_stats},_\S{}\3disk\3\SE{});}}
\L{\LB{\N{9}\V{:}}\Tab{7}{\K{struct}_\V{gendisk}*_\V{disk};}\Tab{32}{\C{}//_block_driver_developers_use_add\_disk(struct_gendisk*)_to_register_disk_into_system\CE{}}}
\L{\LB{\N{10}\V{:}}\Tab{8}{\V{add\_disk}(\V{disk});}}
\index{EOS\_PARAM\_DYN\_CG}\Proc{EOS\_PARAM\_DYN\_CG}\L{\LB{\N{11}\V{:}}\Tab{8}{\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{nr\_requests},_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{\N{12}\V{:}}\Tab{27}{\S{}\3nr\_requests\3\SE{},_\S{}\3disk\3\SE{},_\S{}\3unsigned_long\3\SE{},_\N{64},_\N{4096},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\N{13}\V{:}}\Tab{8}{\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{backing\_dev\_info}.\V{ra\_pages},\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{\N{14}\V{:}}\Tab{27}{\S{}\3ra\_pages\3\SE{},_\S{}\3disk\3\SE{},\S{}\3unsigned_long\3\SE{},_\N{0},_\N{512},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\N{15}\V{:}}\Tab{8}{\V{EOS\_PARAM\_DYN\_FG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{\N{16}\V{:}}\Tab{27}{\S{}\3scheduler\3\SE{},\S{}\3disk\3\SE{},_\S{}\3string\3\SE{},_\S{}\3deadline\3\SE{},\S{}\3deadline:cfq:noop\3\SE{},_\S{}\3\3\SE{},_\&\V{elevator\_change});}}
\L{\LB{\N{17}\V{:}}\Tab{8}{\V{EOS\_PARAM\_DYN\_CG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{\N{18}\V{:}}\Tab{27}{\S{}\3quantum\3\SE{},\S{}\3disk\3\SE{},_\S{}\3unsigned_int\3\SE{},_\N{0},_\N{128},_\S{}\3scheduler=cfq\3\SE{},\&\V{cfq\_quantum\_updater});}}
\L{\LB{\N{19}\V{:}_}}
\L{\LB{\N{20}\V{:}_\K{unsigned}_\K{long}_\V{io\_util}(\K{void})_\{}\Tab{44}{\C{}//_disk_io_utilization\CE{}}}
\L{\LB{\N{21}\V{:}_.\,.\,.}}
\L{\LB{\N{22}\V{:}_\}}}
\L{\LB{\N{23}\V{:}_\V{EOS\_SYSTEM\_UTIL}(\V{io\_util},_\S{}\3disk\3\SE{},_\N{20});}}


==> codes/annotation.cpp.tex <==
% Remember to use the lgrind style

\Head{}
\File{annotation.cpp}{2014}{5}{1}{8:16}{1305}
\L{\LB{\K{struct}_\V{disk\_sensor}_\{}\Tab{27}{\C{}//sensor_representation\CE{}}}
\L{\LB{}\Tab{4}{\K{unsigned}_\K{long}_\V{concurrency};_\K{unsigned}_\K{long}_\V{rw\_ratio};_\K{unsigned}_\K{long}_\V{avg\_io\_size};}}
\L{\LB{}\Tab{4}{\K{unsigned}_\K{long}_\V{avg\_disk\_distance};_\K{unsigned}_\K{long}_\V{avg\_time};_\K{unsigned}_\K{long}_\V{throughput};}}
\L{\LB{\}_\V{DS};}}
\L{\LB{\V{EOS\_SENSOR}_(\V{DS},_\S{}\3disk_20\%:20\%:20\%:50\%:50\%\3\SE{},_\N{6});}}
\index{collect\_disk\_stats}\Proc{collect\_disk\_stats}\L{\LB{\K{void}_\V{collect\_disk\_stats}(\K{void})_\{}\Tab{35}{\C{}//_collect_disk_stats,_calculate_the_signature_and_thoughput_from_last_call_to_now\CE{}}}
\L{\LB{\}}}
\L{\LB{}\Tab{4}{\V{EOS\_STATS\_UPDATER}(\V{collect\_disk\_stats},_\S{}\3disk\3\SE{});}}
\L{\LB{}\Tab{4}{\K{struct}_\V{gendisk}*_\V{disk};}\Tab{29}{\C{}//_block_driver_developers_use_add\_disk(struct_gendisk*)_to_register_disk_into_system\CE{}}}
\L{\LB{}\Tab{4}{\V{add\_disk}(\V{disk});}}
\index{EOS\_PARAM\_DYN\_CG}\Proc{EOS\_PARAM\_DYN\_CG}\L{\LB{}\Tab{4}{\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{nr\_requests},_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{}\Tab{23}{\S{}\3nr\_requests\3\SE{},_\S{}\3disk\3\SE{},_\S{}\3unsigned_long\3\SE{},_\N{64},_\N{4096},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{}\Tab{4}{\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{backing\_dev\_info}.\V{ra\_pages},\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{}\Tab{23}{\S{}\3ra\_pages\3\SE{},_\S{}\3disk\3\SE{},\S{}\3unsigned_long\3\SE{},_\N{0},_\N{512},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{}\Tab{4}{\V{EOS\_PARAM\_DYN\_FG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{}\Tab{23}{\S{}\3scheduler\3\SE{},\S{}\3disk\3\SE{},_\S{}\3string\3\SE{},_\S{}\3deadline\3\SE{},\S{}\3deadline:cfq:noop\3\SE{},_\S{}\3\3\SE{},_\&\V{elevator\_change});}}
\L{\LB{}\Tab{4}{\V{EOS\_PARAM\_DYN\_CG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{}\Tab{23}{\S{}\3quantum\3\SE{},\S{}\3disk\3\SE{},_\S{}\3unsigned_int\3\SE{},_\N{0},_\N{128},_\S{}\3scheduler=cfq\3\SE{},\&\V{cfq\_quantum\_updater});}}
\L{\LB{}}
\L{\LB{\K{unsigned}_\K{long}_\V{io\_util}(\K{void})_\{}\Tab{40}{\C{}//_disk_io_utilization\CE{}}}
\L{\LB{.\,.\,.}}
\L{\LB{\}}}
\L{\LB{\V{EOS\_SYSTEM\_UTIL}(\V{io\_util},_\S{}\3disk\3\SE{},_\N{20});}}


==> codes/api.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{api.cpp.lineno}{2014}{5}{1}{15:36}{1032}
\L{\LB{\N{1}_\V{:}_\K{struct}_\V{eos\_param}_\{}}
\L{\LB{\N{2}_\V{:}}\Tab{8}{\K{const}_\K{char}_*\V{name};_\C{}//_unique_name_of_the_parameter\CE{}}}
\L{\LB{\N{3}_\V{:}}\Tab{8}{\K{const}_\K{char}_*\V{subsys};_\C{}//_the_subsystem_this_parameter_belongs\CE{}}}
\L{\LB{\N{4}_\V{:}}\Tab{8}{\K{unsigned}_\K{long}_\V{min\_value},_\V{max\_value};_\C{}//_value_range\CE{}}}
\L{\LB{\N{5}_\V{:}}\Tab{8}{\K{int}_\V{linear\_or\_exponential\_search};}}
\L{\LB{\N{6}_\V{:}}\Tab{8}{\K{unsigned}_\K{long}_(*\V{getter})(\K{void}_*\V{param});_\C{}//_optional\CE{}}}
\L{\LB{\N{7}_\V{:}}\Tab{8}{\K{void}_(*\V{setter})(\K{void}_*\V{param},_\K{unsigned}_\K{long}_\V{value});_\C{}//_optional\CE{}}}
\L{\LB{\N{8}_\V{:}}\Tab{8}{\K{void}_*\V{param};_\C{}//_where_the_parameter_is_stored_in_memory\CE{}}}
\L{\LB{\N{9}_\V{:}_\};}}
\L{\LB{\N{10}\V{:}_\K{struct}_\V{eos\_guard}_\{}}
\L{\LB{\N{11}\V{:}}\Tab{8}{\K{struct}_\V{eos\_param}_*\V{param};}}
\L{\LB{\N{12}\V{:}}\Tab{8}{\K{unsigned}_\K{long}_\V{value};}}
\L{\LB{\N{13}\V{:}_\};}}
\index{eos\_register\_param}\Proc{eos\_register\_param}\L{\LB{\N{14}\V{:}_\K{void}_\V{eos\_register\_param}(\K{struct}_\V{eos\_param}_*\V{param},}}
\L{\LB{\N{15}\V{:}}\Tab{20}{\K{struct}_\V{eos\_guard}_*\V{guard})}}
\L{\LB{\N{16}\V{:}_}}
\L{\LB{\N{17}\V{:}_\K{struct}_\V{eos\_subsys}_\{}}
\L{\LB{\N{18}\V{:}}\Tab{8}{\K{const}_\K{char}_*\V{name};_\C{}//_unique_name_of_the_subsystem\CE{}}}
\L{\LB{\N{19}\V{:}}\Tab{8}{\K{void}_(*\V{get\_sensors})(\K{int}_\V{size},_\K{unsigned}_\K{long}_*\V{sensors},}}
\L{\LB{\N{20}\V{:}}\Tab{30}{\K{int}_*\V{similarity\_threshold});}}
\L{\LB{\N{21}\V{:}}\Tab{8}{\K{unsigned}_\K{long}_(*\V{get\_optimization\_target})();}}
\L{\LB{\N{22}\V{:}}\Tab{8}{\K{int}_(*\V{is\_bottlenecked})();_\C{}//_returns_zero_unless_bottlenecked\CE{}}}
\L{\LB{\N{23}\V{:}_\};}}
\L{\LB{\N{24}\V{:}_\K{void}_\V{eos\_register\_subsys}(\K{struct}_\V{eos\_subsys}_*\V{subsys});}}


==> codes/cpu_sample.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{cpu\_sample.cpp.lineno}{2014}{5}{1}{8:17}{473}
\L{\LB{\N{1}\V{:}_\K{unsigned}_\K{int}_\V{sysctl\_sched\_latency}_=_\N{6000000ULL};}}
\L{\LB{\N{2}\V{:}_\V{EOS\_PARAM\_CG}(\V{sysctl\_sched\_latency},_\S{}\3scheduler\3\SE{},_\S{}\3unsigned_int\3\SE{},\N{1000000},_\N{1000000000},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\N{3}\V{:}_\K{unsigned}_\K{int}_\V{sysctl\_sched\_min\_granularity}_=_\N{750000ULL};}}
\L{\LB{\N{4}\V{:}_\V{EOS\_PARAM\_CG}(\V{sysctl\_sched\_min\_granularity},_\S{}\3scheduler\3\SE{},\S{}\3unsigned_int\3\SE{},_\N{100000},_\N{1000000000},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\N{5}\V{:}_\K{unsigned}_\K{int}_\V{sysctl\_sched\_wakeup\_granularity}_=_\N{1000000ULL};}}
\L{\LB{\N{6}\V{:}_\V{EOS\_PARAM\_CG}(\V{sysctl\_sched\_wakeup\_granularity},_\S{}\3scheduler\3\SE{},\S{}\3unsigned_int\3\SE{},_\N{100000},_\N{1000000000},_\S{}\3\3\SE{},_\N{0});}}


==> codes/cpu_sample.cpp.tex <==
% Remember to use the lgrind style

\Head{}
\File{cpu\_sample.cpp}{2014}{5}{1}{8:15}{455}
\L{\LB{\K{unsigned}_\K{int}_\V{sysctl\_sched\_latency}_=_\N{6000000ULL};}}
\L{\LB{\V{EOS\_PARAM\_CG}(\V{sysctl\_sched\_latency},_\S{}\3scheduler\3\SE{},_\S{}\3unsigned_int\3\SE{},\N{1000000},_\N{1000000000},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\K{unsigned}_\K{int}_\V{sysctl\_sched\_min\_granularity}_=_\N{750000ULL};}}
\L{\LB{\V{EOS\_PARAM\_CG}(\V{sysctl\_sched\_min\_granularity},_\S{}\3scheduler\3\SE{},\S{}\3unsigned_int\3\SE{},_\N{100000},_\N{1000000000},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\K{unsigned}_\K{int}_\V{sysctl\_sched\_wakeup\_granularity}_=_\N{1000000ULL};}}
\L{\LB{\V{EOS\_PARAM\_CG}(\V{sysctl\_sched\_wakeup\_granularity},_\S{}\3scheduler\3\SE{},\S{}\3unsigned_int\3\SE{},_\N{100000},_\N{1000000000},_\S{}\3\3\SE{},_\N{0});}}


==> codes/disk_sample.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{disk\_sample.cpp.lineno}{2014}{5}{1}{8:17}{1321}
\L{\LB{\N{1}\V{:}_\K{struct}_\V{disk\_sensor}_\{}\Tab{28}{\C{}//sensor_representation\CE{}}}
\L{\LB{\N{2}\V{:}}\Tab{7}{\K{unsigned}_\K{long}_\V{concurrency};_\K{unsigned}_\K{long}_\V{rw\_ratio};_\K{unsigned}_\K{long}_\V{avg\_io\_size};}}
\L{\LB{\N{3}\V{:}}\Tab{7}{\K{unsigned}_\K{long}_\V{avg\_disk\_distance};_\K{unsigned}_\K{long}_\V{avg\_time};_\K{unsigned}_\K{long}_\V{throughput};}}
\L{\LB{\N{4}\V{:}_\}_\V{DS};}}
\L{\LB{\N{5}\V{:}_}}
\L{\LB{\N{6}\V{:}_\V{EOS\_SENSOR}_(\V{DS},_\S{}\3disk_20\%:20\%:20\%:50\%:50\%\3\SE{},_\N{6});}}
\index{collect\_disk\_stats}\Proc{collect\_disk\_stats}\L{\LB{\N{7}\V{:}_\K{void}_\V{collect\_disk\_stats}(\K{void})_\{.\,.\,.\}_\C{}//_collect_disk_stats,_calculate_the_signature_and_thoughput_from_last_call_to_now\CE{}}}
\L{\LB{\N{8}\V{:}_\V{EOS\_STATS\_UPDATER}(\V{collect\_disk\_stats},_\S{}\3disk\3\SE{});}}
\L{\LB{\N{9}\V{:}_}}
\L{\LB{\N{10}\V{:}_\K{struct}_\V{gendisk}*_\V{disk};}\Tab{29}{\C{}//_block_driver_developers_use_add\_disk(struct_gendisk*)_to_register_disk_into_system\CE{}}}
\L{\LB{\N{11}\V{:}_\V{add\_disk}(\V{disk});}}
\index{EOS\_PARAM\_DYN\_CG}\Proc{EOS\_PARAM\_DYN\_CG}\L{\LB{\N{12}\V{:}_\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{nr\_requests},_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{\N{13}\V{:}}\Tab{20}{\S{}\3nr\_requests\3\SE{},_\S{}\3disk\3\SE{},_\S{}\3unsigned_long\3\SE{},_\N{64},_\N{4096},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\N{14}\V{:}_\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{backing\_dev\_info}.\V{ra\_pages},_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{\N{15}\V{:}}\Tab{19}{\S{}\3ra\_pages\3\SE{},_\S{}\3disk\3\SE{},_\S{}\3unsigned_long\3\SE{},_\N{0},_\N{512},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\N{16}\V{:}_\V{EOS\_PARAM\_DYN\_FG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},_\S{}\3scheduler\3\SE{},_\S{}\3disk\3\SE{},}}
\L{\LB{\N{17}\V{:}}\Tab{19}{\S{}\3string\3\SE{},_\S{}\3deadline\3\SE{},_\S{}\3deadline:cfq:noop\3\SE{},_\S{}\3\3\SE{},_\&\V{elevator\_change});}}
\L{\LB{\N{18}\V{:}_\V{EOS\_PARAM\_DYN\_CG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},_\S{}\3quantum\3\SE{},_\S{}\3disk\3\SE{},}}
\L{\LB{\N{19}\V{:}}\Tab{19}{\S{}\3unsigned_int\3\SE{},_\N{0},_\N{128},_\S{}\3scheduler=cfq\3\SE{},_\&\V{cfq\_quantum\_updater});}}
\L{\LB{\N{20}\V{:}_\K{unsigned}_\K{long}_\V{io\_util}(\K{void})_\{.\,.\,.\}}\Tab{46}{\C{}//_disk_io_utilization\CE{}}}
\L{\LB{\N{21}\V{:}_\V{EOS\_SYSTEM\_UTIL}(\V{io\_util},_\S{}\3disk\3\SE{},_\N{20});}}


==> codes/disk_sample.cpp.tex <==
% Remember to use the lgrind style

\Head{}
\File{disk\_sample.cpp}{2014}{5}{1}{8:17}{1246}
\L{\LB{\K{struct}_\V{disk\_sensor}_\{}\Tab{25}{\C{}//sensor_representation\CE{}}}
\L{\LB{}\Tab{4}{\K{unsigned}_\K{long}_\V{concurrency};_\K{unsigned}_\K{long}_\V{rw\_ratio};_\K{unsigned}_\K{long}_\V{avg\_io\_size};}}
\L{\LB{}\Tab{4}{\K{unsigned}_\K{long}_\V{avg\_disk\_distance};_\K{unsigned}_\K{long}_\V{avg\_time};_\K{unsigned}_\K{long}_\V{throughput};}}
\L{\LB{\}_\V{DS};}}
\L{\LB{}}
\L{\LB{\V{EOS\_SENSOR}_(\V{DS},_\S{}\3disk_20\%:20\%:20\%:50\%:50\%\3\SE{},_\N{6});}}
\index{collect\_disk\_stats}\Proc{collect\_disk\_stats}\L{\LB{\K{void}_\V{collect\_disk\_stats}(\K{void})_\{.\,.\,.\}_\C{}//_collect_disk_stats,_calculate_the_signature_and_thoughput_from_last_call_to_now\CE{}}}
\L{\LB{\V{EOS\_STATS\_UPDATER}(\V{collect\_disk\_stats},_\S{}\3disk\3\SE{});}}
\L{\LB{}}
\L{\LB{\K{struct}_\V{gendisk}*_\V{disk};}\Tab{25}{\C{}//_block_driver_developers_use_add\_disk(struct_gendisk*)_to_register_disk_into_system\CE{}}}
\L{\LB{\V{add\_disk}(\V{disk});}}
\index{EOS\_PARAM\_DYN\_CG}\Proc{EOS\_PARAM\_DYN\_CG}\L{\LB{\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{nr\_requests},_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{}\Tab{16}{\S{}\3nr\_requests\3\SE{},_\S{}\3disk\3\SE{},_\S{}\3unsigned_long\3\SE{},_\N{64},_\N{4096},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\V{EOS\_PARAM\_DYN\_CG}(\V{disk}\-\!\>\V{queue}\-\!\>\V{backing\_dev\_info}.\V{ra\_pages},_\V{disk}\-\!\>\V{disk\_name},}}
\L{\LB{}\Tab{15}{\S{}\3ra\_pages\3\SE{},_\S{}\3disk\3\SE{},_\S{}\3unsigned_long\3\SE{},_\N{0},_\N{512},_\S{}\3\3\SE{},_\N{0});}}
\L{\LB{\V{EOS\_PARAM\_DYN\_FG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},_\S{}\3scheduler\3\SE{},_\S{}\3disk\3\SE{},}}
\L{\LB{}\Tab{15}{\S{}\3string\3\SE{},_\S{}\3deadline\3\SE{},_\S{}\3deadline:cfq:noop\3\SE{},_\S{}\3\3\SE{},_\&\V{elevator\_change});}}
\L{\LB{\V{EOS\_PARAM\_DYN\_CG}(*(\V{disk}\-\!\>\V{queue}),_\V{disk}\-\!\>\V{disk\_name},_\S{}\3quantum\3\SE{},_\S{}\3disk\3\SE{},}}
\L{\LB{}\Tab{15}{\S{}\3unsigned_int\3\SE{},_\N{0},_\N{128},_\S{}\3scheduler=cfq\3\SE{},_\&\V{cfq\_quantum\_updater});}}
\L{\LB{\K{unsigned}_\K{long}_\V{io\_util}(\K{void})_\{.\,.\,.\}}\Tab{42}{\C{}//_disk_io_utilization\CE{}}}
\L{\LB{\V{EOS\_SYSTEM\_UTIL}(\V{io\_util},_\S{}\3disk\3\SE{},_\N{20});}}


==> codes/lock_sample.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{lock\_sample.cpp.lineno}{2014}{5}{1}{8:17}{186}
\L{\LB{\N{1}\V{:}_\K{int}_\V{val\_tuner}_=_\N{0};}}
\index{EOS\_PARAM\_CG}\Proc{EOS\_PARAM\_CG}\L{\LB{\N{2}\V{:}_\V{EOS\_PARAM\_CG}(\V{val\_tuner},_\S{}\3lock\3\SE{},_\S{}\3int\3\SE{},_\N{0},_\N{2048},}}
\L{\LB{\N{3}\V{:}_}\Tab{8}{\S{}\3method\_tuner:2\3\SE{},_\N{0});}}
\L{\LB{\N{4}\V{:}_\K{int}_\V{method\_tuner}_=_\N{0};}}
\L{\LB{\N{5}\V{:}_\V{EOS\_PARAM\_FG}(\V{method\_tuner},_\S{}\3lock\3\SE{},_\S{}\3int\3\SE{},}}
\L{\LB{\N{6}\V{:}_\N{0},_\N{2},_\S{}\3\3\SE{},_\N{0});}}


==> codes/lock_sample.cpp.tex <==
% Remember to use the lgrind style

\Head{}
\File{lock\_sample.cpp}{2014}{5}{1}{8:17}{168}
\L{\LB{\K{int}_\V{val\_tuner}_=_\N{0};}}
\index{EOS\_PARAM\_CG}\Proc{EOS\_PARAM\_CG}\L{\LB{\V{EOS\_PARAM\_CG}(\V{val\_tuner},_\S{}\3lock\3\SE{},_\S{}\3int\3\SE{},_\N{0},_\N{2048},}}
\L{\LB{}\Tab{8}{\S{}\3method\_tuner:2\3\SE{},_\N{0});}}
\L{\LB{\K{int}_\V{method\_tuner}_=_\N{0};}}
\L{\LB{\V{EOS\_PARAM\_FG}(\V{method\_tuner},_\S{}\3lock\3\SE{},_\S{}\3int\3\SE{},}}
\L{\LB{\N{0},_\N{2},_\S{}\3\3\SE{},_\N{0});}}


==> codes/memory_imp.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{memory\_imp.cpp.lineno}{2014}{5}{1}{18:59}{1163}
\L{\LB{\N{1}\V{:}_\K{const}_\K{struct}_\V{pr\_policy}_\V{arc\_pr\_policy}_=_\{}}
\L{\LB{\N{2}\V{:}_\C{}/*_Initialize_the_structures._*/\CE{}}}
\L{\LB{\N{3}\V{:}}\Tab{5}{.\V{init\_lruvec}_=_\V{init\_lruvec\_arc},}}
\L{\LB{\N{4}\V{:}_}}
\L{\LB{\N{5}\V{:}_\C{}/*_Decide_which_pages_to_reclaim_and_do_the_reclaiming._*/\CE{}}}
\L{\LB{\N{6}\V{:}}\Tab{5}{.\V{get\_scan\_count}_=_\V{get\_scan\_count\_arc},}}
\L{\LB{\N{7}\V{:}}\Tab{5}{.\V{shrink\_lruvec}_=_\V{shrink\_lruvec\_arc},}}
\L{\LB{\N{8}\V{:}}\Tab{5}{.\V{balance\_lruvec}_=_\V{balance\_lruvec\_arc},}}
\L{\LB{\N{9}\V{:}_}}
\L{\LB{\N{10}\V{:}}\Tab{6}{.\V{should\_continue\_reclaim}_=_\V{should\_continue\_reclaim\_arc},}}
\L{\LB{\N{11}\V{:}}\Tab{6}{.\V{too\_many\_isolated\_compaction}=\V{too\_many\_isolated\_compaction\_arc},}}
\L{\LB{\N{12}\V{:}_}\Tab{8}{}}
\L{\LB{\N{13}\V{:}_\C{}/*_Capture_activity_and_statistics_*/\CE{}}}
\L{\LB{\N{14}\V{:}}\Tab{6}{.\V{page\_accessed}_=_\V{page\_accessed\_arc},}}
\L{\LB{\N{15}\V{:}}\Tab{6}{.\V{activate\_page}_=_\V{activate\_page\_arc},}}
\L{\LB{\N{16}\V{:}}\Tab{6}{.\V{deactivate\_page}_=_\V{deactivate\_page\_arc},}}
\L{\LB{\N{17}\V{:}}\Tab{6}{.\V{update\_pr\_statistics}_=_\V{update\_pr\_statistics\_arc},}}
\L{\LB{\N{18}\V{:}_}}
\L{\LB{\N{19}\V{:}_\C{}/*_Add/release_pages_from_the_LRU_lists._*/\CE{}}}
\L{\LB{\N{20}\V{:}}\Tab{6}{.\V{add\_page}_=_\V{add\_page\_arc},}}
\L{\LB{\N{21}\V{:}}\Tab{6}{.\V{release\_page}_=_\V{release\_page\_arc},}}
\L{\LB{\N{22}\V{:}_}}
\L{\LB{\N{23}\V{:}_\C{}/*_Helpers_used_for_specific_scenarios._*/\CE{}}}
\L{\LB{\N{24}\V{:}}\Tab{6}{.\V{rotate\_inactive\_page}_=_\V{rotate\_inactive\_page\_arc},}}
\L{\LB{\N{25}\V{:}}\Tab{6}{.\V{reset\_zone\_vmstat}_=_\V{reset\_zone\_vmstat\_arc},}}
\L{\LB{\N{26}\V{:}_}}
\L{\LB{\N{27}\V{:}_\C{}/*For_nonresident_lists*/\CE{}}}
\L{\LB{\N{28}\V{:}}\Tab{6}{.\V{nonres\_remember}_=_\V{nonres\_remember\_arc},}}
\L{\LB{\N{29}\V{:}}\Tab{6}{.\V{nonres\_forget}_=_\V{nonres\_forget\_arc},}}
\L{\LB{\N{30}\V{:}}\Tab{6}{.\V{isolate}_=_\V{isolate\_arc},}}
\L{\LB{\N{31}\V{:}}\Tab{6}{.\V{putback\_page}_=_\V{putback\_page\_arc},}}
\L{\LB{\N{32}\V{:}_\};}}


==> codes/memory_sample.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{memory\_sample.cpp.lineno}{2014}{5}{1}{8:17}{163}
\L{\LB{\N{1}\V{:}_\K{const}_\K{char}*_\V{name\_array}[\N{3}]_=_\{\S{}\3LRU2Q\3\SE{},_\S{}\3ARC\3\SE{},_\S{}\3CART\3\SE{}\};}}
\L{\LB{\N{2}\V{:}_\K{int}_\V{mm\_name}_=_\N{0};}}
\index{EOS\_PARAM\_FG}\Proc{EOS\_PARAM\_FG}\L{\LB{\N{3}\V{:}_\V{EOS\_PARAM\_FG}(\V{mm\_name},_\S{}\3memory\3\SE{},_\S{}\3int\3\SE{},}}
\L{\LB{\N{4}\V{:}}\Tab{16}{\N{0},_\N{2},_\S{}\3\3\SE{},_\&\V{memory\_updater});}}


==> codes/memory_sample.cpp.tex <==
% Remember to use the lgrind style

\Head{}
\File{memory\_sample.cpp}{2014}{5}{1}{8:17}{151}
\L{\LB{\K{const}_\K{char}*_\V{name\_array}[\N{3}]_=_\{\S{}\3LRU2Q\3\SE{},_\S{}\3ARC\3\SE{},_\S{}\3CART\3\SE{}\};}}
\L{\LB{\K{int}_\V{mm\_name}_=_\N{0};}}
\index{EOS\_PARAM\_FG}\Proc{EOS\_PARAM\_FG}\L{\LB{\V{EOS\_PARAM\_FG}(\V{mm\_name},_\S{}\3memory\3\SE{},_\S{}\3int\3\SE{},}}
\L{\LB{}\Tab{13}{\N{0},_\N{2},_\S{}\3\3\SE{},_\&\V{memory\_updater});}}


==> codes/spinlock.cpp.lineno.tex <==
% Remember to use the lgrind style

\Head{}
\File{spinlock.cpp.lineno}{2014}{5}{1}{8:14}{302}
\L{\LB{\N{1}\V{:}_\K{struct}_\V{spinlock\_t}_\{}}
\L{\LB{\N{2}\V{:}}\Tab{7}{\K{int}_\V{current};}}
\L{\LB{\N{3}\V{:}}\Tab{7}{\K{int}_\V{next};}}
\L{\LB{\N{4}\V{:}_\};}}
\L{\LB{\N{5}\V{:}_}}
\index{spin\_lock}\Proc{spin\_lock}\L{\LB{\N{6}\V{:}_\K{void}_\V{spin\_lock}(\V{spinlock\_t}_*\V{lock})_\{}}
\L{\LB{\N{7}\V{:}}\Tab{7}{\K{int}_\V{t}=\V{fetch\_and\_inc}(\&\V{lock}\-\!\>\V{next});}}
\L{\LB{\N{8}\V{:}}\Tab{7}{\K{while}_(\V{t}_!=_\V{lock}\-\!\>\V{current})}}
\L{\LB{\N{9}\V{:}}\Tab{11}{\V{pause}(\V{C}*(\V{t}_\-_\V{lock}\-\!\>\V{current}));}}
\L{\LB{\N{10}\V{:}_\}}}
\index{spin\_unlock}\Proc{spin\_unlock}\L{\LB{\N{11}\V{:}_\K{void}_\V{spin\_unlock}(\V{spinlock\_t}_*\V{lock})_\{}}
\L{\LB{\N{12}\V{:}}\Tab{8}{\V{lock}\-\!\>\V{current}++;}}
\L{\LB{\N{13}\V{:}_\}}}


==> cpu_sample.tex <==
%\begin{figure*}
%\lstset{float, language={[ANSI]C}, basicstyle=\ttfamily} %basicstyle=\scriptsize\tt}
%\begin{lstlisting}
%unsigned int sysctl_sched_latency = 6000000ULL;
%EOS_PARAM_CG(sysctl_sched_latency, "scheduler", "unsigned int", 1000000, 1000000000, "", 0);

%unsigned int sysctl_sched_min_granularity = 750000ULL;
%EOS_PARAM_CG(sysctl_sched_min_granularity, "scheduler", "unsigned int", 100000, 1000000000, "", 0);

%unsigned int sysctl_sched_wakeup_granularity = 1000000ULL;
%EOS_PARAM_CG(sysctl_sched_wakeup_granularity, "scheduler", "unsigned int", 100000, 1000000000, "", 0);

%\end{lstlisting}
%\caption{Parameter specifications for CPU scheduling subsystem. Parts of the parameter path 
%are omitted to make the figure fit into the page.}
%\label{spec:cpu}
%\end{figure*}

\begin{figure*}[t]
\centering
%\begin{minipage}{.5\textwidth}
\lgrindfile{codes/cpu_sample.cpp}
%\end{minipage}
\caption{Parameter specifications for CPU scheduling subsystem. Parts of the parameter path 
are omitted to make the figure fit into the page.}
\label{spec:cpu}
\end{figure*}


==> cpu_sig.tex <==
\begin{table}[t]
\center
\caption{Metrics used to represent the signature and throughput in the CPU scheduling subsystem.}{
\label{sigcpu}
\begin{tabular}{|c|c|}
\hline 
\textbf{Purpose} & \textbf{Metrics} \\ 
\hline
\textsc{signature} & \multirow{2}{*}{user space instructions per second} \\ \cline{1-1}
\textsc{throughput} & \\ \hline 
\end{tabular}}
\end{table}


==> design.tex <==
% \section{Example}\label{design}

%% Figure~\ref{overview} presents the architecture of \xxx. While kernel
%% developers are building their kernel, they can use \xxx's API to annotate
%% the policies and parameters in their kernel.  Once the kernel is compiled
%% and distributed, users can run \xxx to tune the parameters and get better
%% performance for their workloads.

\input{example.tex}

We use the disk I/O as an example to show how the system works (Figure~\ref{example} 
presents the sample code). Assume we want to 
tune parameters in the disk IO subsystem to acquire better performance. Thus, 
to use eos, the kernel developer needs to do two things. First, the developer should 
specify tunable parameters using eos APIs. Basically, the block driver needs to call 
the function \texttt{add\_disk (struct gendisk*)} to register each disk into the system. 
After that, developer may call the function \texttt{eos\_register\_param (struct eos\_param*, 
struct eos\_guard*)} to add one tunable parameter. From the first parameter, one can find
information such as the address of this parameter, its name, the subsystem it belongs to, 
minimal value and maximal value, etc. Second, the kernel developer needs to register the 
subsystem using \texttt{eos\_register\_subsys (struct eos\_subsys*)} function. 
Basically, from the function call, we can acquire a set of sensors which capture the 
subsystem bahviour, the system throughput function and the utilization function.  
 
For user side, it needs to insert an auto-tuning module. This module can use 
the utilization function that provided by the developer to decide whether the 
target subsystem is bottleneck. If it is, our tuning module can tune the parameters
based on the parameter specification that is provided by the kernel developer. 
If the workload needs a long time to execute, we can cache the optimial parameters
in the policy cache and reuse them when a similar workload has been executed before.

%\input{annotation.tex}
 
%Because our system is self-adaptive 
%operating system, the classical observation, decision and action (i.e., ODA) loop can be 
%used here~\cite{oda} to understand our system. Specifically, in the ODA loop, the observation part 
%monitors a set of events in the system, which we are interested in; the decision determines which policy 
%to use or whether policy switching is necessary based on the collected information; the action part finally 
%enforces the preferred policy into the system. Corresponding to our system, software sensors are placed into 
%the kernel to collect metrics to represent application signatures or approximate throughput. This process
%can be considered as monitoring. Then, collected information are used to index the \textsc{policy cache}.
%If there is a cache hit, which means exactly the same application or a similar application has been
%executed before, the cached (optimal) parameters are enforced directly into the system. Or else (\textsc{policy 
%cache} misses), we resort to the \textsc{search engine} to find the optimal set of parameters and enforce these
%parameters. Thus, \textsc{policy cache} and \textsc{search engine} in our system are responsible for 
%decision and action parts of the ODA loop.       

%% \subsection{Kernel Extensions}
%% The operating system are extended for two purposes (corresponding to the two hexagons in 
%% Figure~\ref{overview}). One is to expose information of the system by the use of software sensors. 
%% The exposed information are used to approximate throughput of a subsystem and characterize an application. 
%% In our system, approximating throughput is required because the \textsc{search engine} needs to evaluate the 
%% performance of a policy setting to drive the search, while characterizing application is necessary because 
%% the \textsc{policy cache} needs the application signature to identify whether the optimal parameters have been 
%% cached or not. So, a question is which system statistics are needed? Actually, this question is hard 
%% to answer in general because different subsystems usually need different information. In this section, we only 
%% provide the guideline in high level. In Section~\ref{eval}, one can find the concrete metrics for specific 
%% subsystems. For information targeting to represent the throughput of a subsystem, the metric should be able to 
%% quantify the operations of this subsystem on hardware or software resources. 
%% Because the operating system is used to manage resources, if a metric is able to measure the efficiency of 
%% a subsystem on its managed resources, the metric can be used as the throughput of this subsystem.
%% Taking the CPU scheduler as an example, the managed resources of the scheduler is CPU, which are responsible 
%% for executing instructions. Thus, the number of instructions per cycle (i.e., IPC) seems a good metric to 
%% quantify the CPU scheduling subsystem. For the synchronization in the operating system, resources are 
%% locks, so the number of lock acquisitions in a fixed time is a reasonable metric. 
%% For the system information used as application signature, they should be able to capture the characteristics 
%% of the target subsystem when executing an application. Thus, applications with different subsystem characteristics
%% should have different application signatures. Besides, application with different subsystem characteristics 
%% at different execution stage should have different signatures. In theory, the application signatures should 
%% contain enough information such that combining with system parameters as inputs, one can construct an 
%% analytic model to calculate the subsystem throughput.     
%% After determining exposed information, kernel developers need to add routines in the kernel to collect 
%% and make them updated regularly. EOS provides APIs (EOS\_SENSOR\_THP and EOS\_SENSOR\_SIG) to acquire throughput 
%% and signature results, respectively.

%% The second purpose of kernel extensions is to integrate multiple implementations in each target subsystem. 
%% Although Linux has designed in this way for some subsystem (e.g., disk scheduler), most subsystems still adopt 
%% the \textit{one-size-fits-all} design. For instance, Linux uses ticket spin lock as the basic synchronization 
%% method, which is only effective in middle level contention, but in the real world, the contention degree 
%% varies significantly, which may introduce suboptimal performance. To overcome this disadvantage, for each 
%% target subsystem, we integrate policies optimized for different conditions. Besides, we provide a mechanism 
%% to switch to a different policy dynamically. Note that an efficient switching mechanism between different 
%% implementations is usually not trivial.        

%% \input{auto.tex}

%% \subsection{Auto-tuning Module}
%% A kernel module is designed and implemented to optimize the system performance based on the developer 
%% provided parameter specification. This modules has two running modes, which are online mode and offline mode.
%% Specifically, the online mode diagnoses the bottleneck subsystem first before auto-tuning the target 
%% application, while offline mode does not invoke bottleneck searching logic and module users should pass 
%% the bottleneck subsystem as a parameter. The offline mode can expose the maximal performance improvement
%% potential given the bottleneck subsystem. 
%% In the offline mode, one needs to write \texttt{enable} and \texttt{disable} to \texttt{/proc/fast\_auto} 
%% before and after the execution of the target application. When \texttt{enable} is written, we create a kernel 
%% thread at background to perform the parameter tuning. The logic is presented in Algorithm~\ref{aa}. As 
%% we can see, the kernel thread uses \textsc{search engine} to generate all parameter 
%% settings and evaluate them one by one (line $7$). After evaluating the first parameter setting,
%% we use application signatures which are collected when evaluating
%% the first parameter setting to index the \textsc{policy cache} (line $10$). If there is a cache hit, 
%% we acquire the optimal parameter settings from the cache and enforce them to the system directly (line $17$), 
%% or else, we resort to \textsc{search engine} to look for the optimal parameter settings. 
%% The auto-tuning module is made up of three parts, including \textsc{parser}, \textsc{search engine} 
%% and \textsc{policy cache}. Each part will be detailed in following sections.

%% \input{admin}
%% \subsubsection{Profiler}
%% Algorithm~\ref{admin} presents the logic used by the profiler. Because the developer of each kernel 
%% subsystem already provides the way of measuring subsystem utilization (by the use of EOS\_SENSOR\_UTIL API), 
%% which is visible to our kernel module. The profiler uses these functions one by one to decide which subsystem 
%% is intensively used. Basically, we try each registered subsystem. If the utilization of a particular subsystem 
%% is larger than a threshold (also provided as a parameter in the API), we consider this subsystem is intensive 
%% and will use sensor APIs of that subsystem in the auto-tuning phase. 

%% \subsubsection{Parser}
%% \textsc{Parser} used to analyze the kernel developer provided parameter information and transfer it to 
%% the input of \textsc{search engine}. Recall that kernel developers use EOS\_PARAM\_* macro to annotate 
%% a parameter. Basically, the effect of this macro is to add the information of this parameter to a special 
%% section in the kernel, which are visible to our kernel module. At the time of inserting the kernel module,
%% the parser analyses the information in the special kernel section and transfers them into internal 
%% representations. Specifically, each parameter described in the specification is abstracted as a dimension in 
%% the $N$-dimension parameter space, where $N$ is the number of parameters. In our implementation, the dimension 
%% is programmed as a \texttt{struct} and parameter related information such as type, range, etc are different 
%% domains in this \texttt{struct}. All parameters form a parameter space and we use a \texttt{struct} array 
%% with dynamic size to represent it.  

%% \input{search.tex}
%% \input{policy}

%% \subsubsection{Searching Engine}

%% \textsc{Search engine} is exploited to find the optimal parameter settings for the target application. 
%% As presented in Figure~\ref{aa}, it takes the output of \textsc{parser} as input and generates one 
%% parameter setting at each search step. The length of each step lasts five seconds. At the end of each step, 
%% the kernel thread in the auto-tuning module collects the evaluation results of the target subsystem 
%% with the current parameter setting and feed the results into \textsc{search engine} to switch to next 
%% parameter setting. The search process continues until all parameter settings are evaluated. Then, 
%% the parameter settings with the largest throughput are enforced to the subsystem. Note that users of our 
%% system can use any preferred parameter search algorithm in the framework. To show the effectiveness of 
%% auto-tuning and parameter caching, our current implementation is the enhanced orthogonal search~\cite{atlas} 
%% (we modify the logic based on our context). Specifically, the global optimal parameter settings are 
%% approximated using the optimal parameter setting at each dimension. Given all parameters that are worth 
%% tuning, they can be divided into two classes. One is called independent class, where there is no dependency 
%% for any two parameters. The other is dependent class, 
%% where each parameter depends on one or several parameters in the independent class. 
%% Note that the dependency between parameters can be acquired from the parameter specification (see 
%% Section~\ref{spec}). Our search begins in the independent parameter class. After assigning a value 
%% of each parameter in this class, parameters in the dependent class are checked to enable parameters 
%% that satisfy parameter dependencies. 
%% Besides, in our \textsc{search engine}, a parameter with \texttt{method} property has higher priority 
%% than a parameter with \texttt{value} property because \texttt{method} parameters tend to have fewer possible 
%% values and larger impact on operating system performance. To take this factor into consideration, our
%% \textsc{search engine} finds the optimal parameter setting for \texttt{method} parameters first and 
%% then searches optimal value for \texttt{value} parameters (line $15$ to $22$ in Algorithm~\ref{as}). 
%% Note that when a parameter has property \texttt{value}, but type \texttt{int}, the range of the parameter 
%% could be large and it is impossible to evaluate each value. To cope with this situation, there is a tuning 
%% step in the parameter specification, our \textsc{search engine} can use developer suggested step to increase 
%% a parameter. Besides, we can also configure the \textsc{search engine} to ignore the developer provided 
%% linear step and use an exponential tuning step. Our experimental results in Section~\ref{eval} use the latter.    

%% The \textsc{search engine} has the capability of restarting the search after finding the optimal parameter 
%% settings already (line $2$ to $4$). Specifically, we keep monitoring the system throughput until it changes 
%% significantly (much larger or smaller than the results of the best setting). Besides, the tuning is also 
%% restarted periodically.  
    

%\input{policy}



==> design_backup.tex <==
\section{Design and Implementation}
\label{design}

\input{overview}
\subsection{Overview}
Figure~\ref{overview} presents the software architecture of EOS. Because our system is self-adaptive 
operating system, the classical observation, decision and action (i.e., ODA) loop can be 
used here~\cite{oda} to understand our system. Specifically, in the ODA loop, the observation part 
monitors a set of events in the system, which we are interested in; the decision determines which policy 
to use or whether policy switching is necessary based on the collected information; the action part finally 
enforces the preferred policy into the system. Corresponding to our system, software sensors are placed into 
the kernel to collect metrics to represent application signatures or approximate throughput. This process
can be considered as monitoring. Then, collected information are used to index the \textsc{policy cache}.
If there is a cache hit, which means exactly the same application or a similar application has been
executed before, the cached (optimal) parameters are enforced directly into the system. Or else (\textsc{policy 
cache} misses), we resort to the \textsc{search engine} to find the optimal set of parameters and enforce these
parameters. Thus, \textsc{policy cache} and \textsc{search engine} in our system are responsible for 
decision and action parts of the ODA loop.       

\subsection{Parameter Specification}
\label{spec}
EOS can automatically search for optimal value of system parameters for the target application,
but kernel developers should provide parameter specifications of each subsystem when the operating system
is released. The parameter specification details some basic information about each parameter and the
relationship between parameters. Each parameter worth tuning is described by the template,
$<$\texttt{D:parameterID:subsystem:property:location: type:default:range}$>$. In the template, one can
find the subsystem that the parameter belongs to, the location to modify the parameter, the type of the
parameter, the default setting of the parameter, etc. The \texttt{property} domain of a parameter can
be \texttt{method} or \texttt{value}. If it is \texttt{method}, that means the modification of the parameter
value invokes the implementation change of a policy, or else, the parameter is an intrinsic parameter in
the policy implementation. For the type of a parameter, it can be \texttt{enum} or \texttt{int}. If the
type of a parameter is \texttt{enum}, all possible values need to be listed in the \texttt{range} domain,
separate by commas, or else, the minimal value,  maximal value and recommended tuning step of this variable
are provided in \texttt{range}.

Besides, dependences of different parameters are also described in the parameter specification.
This information is needed because parameters of an algorithm are worth to tune only when this
algorithm is enabled in the system. By considering the parameter dependences, the work of auto-tuning
can be significantly reduced. To demonstrate this conclusion, let's us consider an example. Assume there
are two implementations ($I_A$ and $I_B$) for a subsystem. $I_A$ and $I_B$ have $P_A$ and $P_B$ parameters,
respectively. Assume there are $C$ values for each parameter. If we do not consider the fact that
only one implementation takes effects at any time, there will be $C^{P_A + P_B}$ possible parameter value
combinations. However, the large space can be reduced to $C^{P_A}$ or $C^{P_B}$ depending on
which implementation to use. The template used to describe the parameter dependence is
$<$\texttt{R:parameterID$_1$:parameterID$_2$,methodID}$>$, which indicates \texttt{parameterID$_1$} depends
on \texttt{parameterID$_2$} when \texttt{parameterID$_2$} is assigned to \texttt{methodID}. Note that
the quality of a specification does affect the performance of the target application because the searching overhead is
proportional to the number of parameters in the specification. Besides, a specification with casually
selected parameters, parameter range or searching step may cause suboptimal application performance. However,
we believe that the required information of a parameter is very basic for a kernel developer to provide
and will not become a burden of kernel developers. By default, the parameter specification locates at
\texttt{/var/eos/spec}.

\subsection{Kernel Extensions}
The operating system are extended for two purposes (corresponding to the two hexagons in 
Figure~\ref{overview}). One is to expose information of the system by the use of software sensors. 
The exposed information are used to approximate throughput of a subsystem and characterize an application. 
In our system, approximating throughput is required because the \textsc{search engine} needs to evaluate the 
performance of a policy setting to drive the search, while characterizing application is necessary because 
the \textsc{policy cache} needs the application signature to identify whether the optimal parameters have been 
cached or not. So, a question is which system statistics are needed? Actually, this question is hard 
to answer in general because different subsystems usually need different information. In this section, we only 
provide the guideline in high level. In Section~\ref{eval}, one can find the concrete metrics for specific 
subsystems. For information targeting to represent the throughput of a subsystem, the metric should be able to 
quantify the operations of this subsystem on hardware or software resources. 
Because the operating system is used to manage resources, if a metric is able to measure the efficiency of 
a subsystem on its managed resources, the metric can be used as the throughput of this subsystem.
Taking the CPU scheduler as an example, the managed resources of the scheduler is CPU, which are responsible 
for executing instructions. Thus, the number of instructions per cycle (i.e., IPC) seems a good metric to 
quantify the CPU scheduling subsystem. For the synchronization in the operating system, resources are 
locks, so the number of lock acquisitions in a fixed time is a reasonable metric. 
For the system information used as application signature, they should be able to capture the characteristics 
of the target subsystem when executing an application. Thus, applications with different subsystem characteristics
should have different application signatures. Besides, application with different subsystem characteristics 
at different execution stage should have different signatures. In theory, the application signatures should 
contain enough information such that combining with system parameters as inputs, one can construct an 
analytic model to calculate the subsystem throughput.     
After determining exposed information, we need to increase routines in the kernel to collect and make them 
updated regularly. Besides, these variables should be accessible by the auto-tuning kernel module. Because 
the kernel and auto-tuning module operate the information via shared memory, one should keep data consistency 
across read and write operations. Also note that the information is read-only in the auto-tuning module and 
write-only at kernel side, thus, optimizations such as \texttt{seqlock}-based synchronization are used.        

The second purpose of kernel extensions is to integrate multiple implementations in each target subsystem. 
Although Linux has designed in this way for some subsystem (e.g., disk scheduler), most subsystems still adopt 
the \textit{one-size-fits-all} design. For instance, Linux uses ticket spin lock as the basic synchronization 
method, which is only effective in middle level contention, but in the real world, the contention degree 
varies significantly, which may introduce suboptimal performance. To overcome this disadvantage, for each 
target subsystem, we integrate policies optimized for different conditions. Besides, we provide a mechanism 
to switch to a different policy dynamically. Note that an efficient switching mechanism between different 
implementations is usually not trivial.        

\input{auto.tex}

\subsection{Auto-tuning Module}
A kernel module is designed and implemented to optimize the system performance based on the developer 
provided parameter specification. To use our module, one needs to write \texttt{enable} and \texttt{disable} 
to \texttt{/proc/fast\_auto} before and after the execution of the target application. When \texttt{enable} 
is written, we create a kernel thread at background to perform the parameter tuning. The logic is presented 
in Algorithm~\ref{aa}. As we can see, the kernel thread uses \textsc{search engine} to generate all parameter 
settings and evaluate them one by one (line $7$). After evaluating the first parameter setting,
we use application signatures which are collected when evaluating
the first parameter setting to index the \textsc{policy cache} (line $10$). If there is a cache hit, 
we acquire the optimal parameter settings from the cache and enforce them to the system directly (line $17$), 
or else, we resort to \textsc{search engine} to look for the optimal parameter settings. 
The auto-tuning module is made up of three parts, including \textsc{parser}, \textsc{search engine} 
and \textsc{policy cache}. Each part will be detailed in following sections.
 
\subsubsection{Parser}
\textsc{Parser} used to analyze the kernel developer provided parameter specification and transfer it to 
the input of \textsc{search engine}. Specifically, each parameter described in the specification is abstracted 
as a dimension in the $N$-dimension parameter space, where $N$ is the number of parameters. In our implementation, 
the dimension is programmed as a \texttt{struct} data structure and parameter related information such as type, 
location, range, etc are different domains in this \texttt{struct}. All parameters form a parameter space and 
we use a \texttt{struct} array with dynamic size to represent it. Our parser supports flexible specification formats. 
One can use comments (each line started with \#) and causal white spaces. Besides, no order constrains are required 
between any two parameter descriptions. 

\input{search.tex}
\input{policy}

\subsubsection{Searching Engine}

\textsc{Search engine} is exploited to find the optimal parameter settings for the target application. 
As presented in Figure~\ref{aa}, it takes the output of \textsc{parser} as input and generates one 
parameter setting at each search step. The length of each step lasts five seconds. At the end of each step, 
the kernel thread in the auto-tuning module collects the evaluation results of the target subsystem 
with the current parameter setting and feed the results into \textsc{search engine} to switch to next 
parameter setting. The search process continues until all parameter settings are evaluated. Then, 
the parameter settings with the largest throughput are enforced to the subsystem. Note that users of our 
system can use any preferred parameter search algorithm in the framework. To show the effectiveness of 
auto-tuning and parameter caching, our current implementation is the enhanced orthogonal search~\cite{atlas} 
(we modify the logic based on our context). Specifically, the global optimal parameter settings are 
approximated using the optimal parameter setting at each dimension. Given all parameters that are worth 
tuning, they can be divided into two classes. One is called independent class, where there is no dependency 
for any two parameters. The other is dependent class, 
where each parameter depends on one or several parameters in the independent class. 
Note that the dependency between parameters can be acquired from the parameter specification (see 
Section~\ref{spec}). Our search begins in the independent parameter class. After assigning a value 
of each parameter in this class, parameters in the dependent class are checked to enable parameters 
that satisfy parameter dependencies. 
Besides, in our \textsc{search engine}, a parameter with \texttt{method} property has higher priority 
than a parameter with \texttt{value} property because \texttt{method} parameters tend to have fewer possible 
values and larger impact on operating system performance. To take this factor into consideration, our
\textsc{search engine} finds the optimal parameter setting for \texttt{method} parameters first and 
then searches optimal value for \texttt{value} parameters (line $15$ to $22$ in Algorithm~\ref{as}). 
Note that when a parameter has property \texttt{value}, but type \texttt{int}, the range of the parameter 
could be large and it is impossible to evaluate each value. To cope with this situation, there is a tuning 
step in the parameter specification, our \textsc{search engine} can use developer suggested step to increase 
a parameter. Besides, we can also configure the \textsc{search engine} to ignore the developer provided 
linear step and use an exponential tuning step. Our experimental results in Section~\ref{eval} use the latter.    

The \textsc{search engine} has the capability of restarting the search after finding the optimal parameter 
settings already (line $2$ to $4$). Specifically, we keep monitoring the system throughput until it changes 
significantly (much larger or smaller than the results of the best setting). Besides, the tuning is also 
restarted periodically.  
    

%\input{policy}
\subsubsection{Policy Cache}

\textsc{Policy cache} is used to speedup searching in the parameter space and Algorithm~\ref{ap} presents 
the logic. For a specification with many tunable parameters, the search overhead could be significant. The 
basic idea of \textsc{policy cache} is to store the execution history of an application by the use of 
$<$\texttt{application signature}, \texttt{parameter settings}$>$ pair. When the same application or a similar 
application executes, we enforce the optimal parameter settings directly without searching. The key issue of 
using \textsc{policy cache} is to identify whether a similar application has executed before. This paper uses 
the information collected from the extended kernel as the application signatures. In terms of the algorithm
that judges whether \textsc{policy cache} is hit or not, our framework provides the flexibility to users. 
Basically, users only need to implement \texttt{policy\_cache} and \texttt{put} functions in the framework 
(see Algorithm~\ref{aa}). Using these two interfaces, kinds of caching algorithms can be implemented, even 
complex machine learning algorithms. Our current implementation exploits a simple logic to suggest the idea
of parameter caching. Specifically, we use the vector formed by collected metrics to compare with the stored 
metric vector (line $2$). If each dimension of these two metric vectors are near enough (i.e., within 20\% 
percent), the new application hits the cache.  
One point worth mentioning is that if an application has relatively short execution time, no optimal parameter 
settings are stored in \textsc{policy cache} because the search is not finished yet. In this case, we also 
store the metric vector as before at the time of application termination, but we tag the cached element 
with \textit{uncompleted} (line $26$ in Algorithm~\ref{aa}). When the same application is executed again, 
the stored metrics are used to initialize the execution (line $12$ in Algorithm~\ref{aa}). 
Note that the content of \textsc{policy cache} is persistent as it is dumped into the \texttt{/var/eos/cache} 
file after the auto-tuning module is removed. When the auto-tuning module is inserted next time, the content 
in the cache file is used to populate \textsc{policy cache}. 

\input{admin}


==> disk_sample.tex <==
%\begin{figure*}[t]
%\lstset{float, language={[ANSI]C}, basicstyle=\ttfamily}%, numbers=left, numberstyle=\tiny}%, basicstyle=\scriptsize\tt}
%\begin{lstlisting}
%//sensor representation
%struct disk_sensor {
%unsigned long concurrency;
%unsigned long rw_ratio;
%unsigned long avg_io_size;
%unsigned long avg_disk_distance;
%unsigned long avg_time;
%unsigned long throughput;
%} DS;
%EOS_SENSOR (DS, "disk 20%:20%:20%:50%:50%", 6);

%void collect_disk_stats(void)
%{
%	// collect disk stats, calculate the signature and thoughput from last call to now
%}
%EOS_STATS_UPDATER(collect_disk_stats, "disk");

%struct gendisk* disk;
%// block driver developers use add_disk(struct gendisk*) to register disk into system
%add_disk(disk);
%EOS_PARAM_DYN_CG(disk->queue->nr_requests, disk->disk_name, "nr_requests", "disk", "unsigned long", 64, 4096, "", 0);
%EOS_PARAM_DYN_CG(disk->queue->backing_dev_info.ra_pages, disk->disk_name, "ra_pages", "disk", "unsigned long", 0, 512, "", 0);
%EOS_PARAM_DYN_FG(*(disk->queue), disk->disk_name, "scheduler", "disk", "string", "deadline", "deadline:cfq:noop", "", &elevator_change);
%EOS_PARAM_DYN_CG(*(disk->queue), disk->disk_name, "quantum", "disk", "unsigned int", 0, 128, "scheduler=cfq", &cfq_quantum_updater);
%unsigned long io_util(void) 
%{
%	// disk io utilization 
%	...
%}
%EOS_SYSTEM_UTIL(io_util, "disk", 20);
%\end{lstlisting}
%\caption{Parameter specifications for disk scheduling subsystem.}
%\label{spec:disk}
%\end{figure*}

\begin{figure*}[t]
\centering
%\begin{minipage}{.5\textwidth}
\lgrindfile{codes/disk_sample.cpp}
%\end{minipage}
\caption{Parameter specifications for disk scheduling subsystem.}
\label{spec:disk}
\end{figure*}

==> hlock.tex <==
\begin{table}
\center
\caption{Hot kernel locks for each benchmark}{
\label{hl}
\begin{tabular}{|l|c|}
  \hline
  \textbf{Benchmarks} & \textbf{Kernel Locks} \\
  \hline \hline  
  \textit{fops} & dentry lock (d\_lock) \\ \hline
  \textit{mmapbench} & mapping mutex (i\_mmap\_mutex) \\ \hline
  \textit{postmark} & file descriptor table lock \\ \hline
  \multirow{4}{2cm}{\textit{dbench}} & dentry lock (d\_lock) \\ \cline{2-2}
  & per CPU counter lock \\ \cline{2-2}
  & inode lock (inode\_sb\_list\_lock) \\ \cline{2-2}
  & tmpfs statistics lock (stat\_lock) \\ \hline
\end{tabular}}
\end{table}




==> ioresults.tex <==
\begin{figure*}[t]
\centering

\subfigure[{SKIP}]
{
   \includegraphics[width=0.45\textwidth]{io/skip.eps}
}
\subfigure[{zmIO}]
{
    \includegraphics[width=0.45\textwidth]{io/zmio.eps}
}
\subfigure[{fsmark}]
{
    \includegraphics[width=0.45\textwidth]{io/fsmark.eps}
}
\subfigure[{sysbench}]
{
   \includegraphics[width=0.45\textwidth]{io/sysbench.eps}
}
\subfigure[{parallel find}]
{
    \includegraphics[width=0.45\textwidth]{io/pfind.eps}
}
\subfigure[{parallel grep}]
{
    \includegraphics[width=0.45\textwidth]{io/pgrep.eps}
}
\subfigure[{TPC-C}]
{
   \includegraphics[width=0.45\textwidth]{io/tpcc.eps}
}
\caption{IO scheduler performance}
\label{fig:io}
\end{figure*}



==> ioschedule-table.tex <==
\begin{table*}[t]
%\scriptsize
\center
\caption{Performance results of stickleback under different benchmarks.
\label{tab1}
AUTO-before presents the cold \textit{policy cache} performance, while AUTO is the 
hot \textit{policy cache} performance. The unit of SKIP, parallel find and parallel 
grep are seconds and the unit of the remaining benchmarks are ops (i.e., operations per 
second).}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
Benchmarks \& methods & DEADLINE & CFQ & NOOP & AUTO-before & AUTO \\ \hline
\hline
$SKIP$     & 954.0 s & 72.1 s & 961.9 s & 84.9 s & 75.0 s \\ \hline 
$zmIO$     & 3038.6 ops & 1965.3 ops & 2294.8 ops & 2702.3 ops & 2980.2 ops \\ \hline
$fsmark$   & 66.1 ops & 71.4 ops & 69.3 ops & 67.6 ops & 73.1 ops \\ \hline
$sysbench$ & 13.0 ops & 13.4 ops & 13.2 ops & 12.6 ops & 12.4 ops \\ \hline 
$pfind$    & 26.6 s & 30.6 s & 26.0 s & 26.3 s & 26.6 s \\ \hline
$pgrep$    & 682.5 s & 229.5 s & 692.0 s & 233.1 s & 227.0 s \\ \hline 
$HammerDB$ & 355853.4 ops & 369368.2 ops & 381202.0 ops & 396355.2 ops & 462901.0 ops \\ \hline
\end{tabular}}
\end{table*}


==> lock_sample.tex <==
%\begin{figure*}[t]
%\lstset{float, language={[ANSI]C}, basicstyle=\ttfamily}%, numbers=left, numberstyle=\tiny} %basicstyle=\tiny\tt}
%\begin{lstlisting}
%int val_tuner = 0;
%EOS_PARAM_CG(val_tuner, "lock", "int", 0, 2048, "method_tuner:2", 0);

%int method_tuner = 0;
%EOS_PARAM_FG(method_tuner, "lock", "int", 0, 2, "", 0);
%\end{lstlisting}
%\caption{Parameter specifications for mixed lock protocol.}
%\label{spec:lock}
%\end{figure*}
\begin{figure}[t]
\centering
%\begin{minipage}{.5\textwidth}
\lgrindfile{codes/lock_sample.cpp}
%\end{minipage}
\caption{Parameter specifications for mixed lock protocol.}
\label{spec:lock}
\end{figure}


==> lock_sig.tex <==
\begin{table}[t]
\center
\caption{Metrics used to represent the signature and throughput in the mixed lock protocol.}{
\label{siglock}
\begin{tabular}{|c|c|}
\hline 
\textbf{Purpose} & \textbf{Metrics} \\ 
\hline
\textsc{signature}  & average lock acquisition time \\ \hline 
\textsc{throughput} & lock acquisitions per second \\ \hline 
\end{tabular}}
\end{table}


==> motpic.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.43\textwidth]{mot}
\caption{Performance of sysbench thread test when using default and tuned parameters.
Y-axes represents execution time. Thus, the smaller the better.}
\label{fig:mot}
\end{figure}



==> policy.tex <==
\begin{algorithm}
\small
\LinesNumbered
\KwIn{policy cache \texttt{perfcache}, signature \texttt{sig}}
\KwOut{index in the policy cache}
\For{\texttt{i} $\gets$ \texttt{perfcache.guard} \textbf{to} \texttt{0}}{
 \If{hit\_cache(\texttt{sig},\texttt{perfcache.perfc[i].sig})}{
  \Return \texttt{i} \; 
 }
}
\Return \texttt{-1} \;
\caption{index\_policy\_cache() function}
\label{ap}
\end{algorithm}


==> prn0.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{PRN_0}
\caption{Performance of MSR traces (PRN0)}  
\label{prn}
\end{figure}


==> sched_params.tex <==
\begin{table*}[t]
\center
\caption{All Tunable Parameters in the Scheduling Subsystem}{
\label{schedparam}
\begin{tabular}{|c|c|c|c|}
\hline 
\textbf{Parameters} & \textbf{Meaning} & \textbf{Range} & \textbf{Tuned} \\ 
\hline \hline
\textbf{sched\_min\_granularity\_ns} & minimal scheduled execution time & positive integers & YES \\ \hline 
\textbf{sched\_latency\_ns} & time for scheduling a group of tasks & positive integers & YES \\ \hline
\textbf{sched\_wakeup\_granularity\_ns} & ability to wake up and preempt the current task & positive integers & YES \\ \hline
sched\_tunable\_scaling & way of adjusting parameter value on SMPs & 0,1,2,3 & NO \\ \hline
sched\_time\_avg\_ms & peorid of averaging the RT time consumption & positive integers & NO \\ \hline
sched\_shares\_window\_ns & window of calculating average load for shares distribution & positive integers & NO \\ \hline
sched\_rt\_runtime\_us & maximal CPU time used by RT tasks & positive integers & NO \\ \hline
sched\_rt\_peorid\_us & time to wait before scheduling a RT task again & positive integers & NO \\ \hline
sched\_nr\_migrate & maximal tasks to migrate during load balancing & positive integers & NO \\ \hline
sched\_migration\_cost\_ns & cost of task migration among CPUs & positive integers & NO \\ \hline
sched\_child\_runs\_first & order of execution between parent and child & 0,1 & NO \\ \hline
sched\_autogroup\_enabled & enable the auto-group feature or not & 0,1 & NO \\ \hline
sched\_cfs\_bandwidth\_slice\_us & cgroup bandwidth control & positive integers & NO \\ \hline
\end{tabular}}
\end{table*}


==> trace.tex <==
\begin{figure}[t]
\centering
\subfigure[{source control server}]
{
   \includegraphics[width=0.45\textwidth]{src1}
}
\subfigure[{file server for researchers}]
{
   \includegraphics[width=0.45\textwidth]{usr0}
}
\caption{Aggregated IO performance for one typical week.}
\label{trace}
\end{figure}



==> trace1.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{src1}
\caption{source control server}  
\label{traces1}
\end{figure}


==> trace2.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{usr0}
\caption{file server}  
\label{traces2}
\end{figure}


==> trace3.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{wdev2}
\caption{web develop server}  
\label{traces3}
\end{figure}

